Attainable Force Approximation and Full-Pose Tracking Control of an Over-Actuated Thrust-Vectoring Modular Team UAV

Traditional vertical take-off and landing (VTOL) aircraft can not achieve optimal efficiency for various payload weights and has limited mobility due to its under-actuation. With the thrust-vectoring mechanism, the proposed modular team UAV is fully actuated at certain attitudes. However, the attainable force space (AFS) differs according to the team configuration, which makes the controller design difficult. We propose an approximation to the AFS and a full-pose tracking controller with an attitude planner and a force projection, which guarantees the control force is feasible. The proposed approach can be applied to UAVs having multiple thrust-vectoring effectors with homogeneous agents. The simulation and experiment demonstrate a tilting motion during hovering for a 4-agent team.

==> contents/control_allocation.tex <==
\section{Exact Bundled Redistributed Control Allocation (EBRCA)}

EBRCA is an extension of  \cite{stephanFastExactRedistributed2019} such that the exact and the direction-preserving concept can be applied to bundled thrust-vectoring subsystems by finding intersections on the bundled AFS.

% Determines the tendency of changes
% The local admissible force space

% by linearizing $\mathbf{f}$, 

% Given the current state, $\mathbf{z}_{i}$, from \eqref{eq:model:team:effectiveness_model}, agents' thrust is $\mathbf{f}_i = {T_f}_i \hat{\mathbf{a}}_i$, and the .

% Given the current state, $\mathbf{f}_{0i}$, and the desired decomposed force vector $\mathbf{f}_{id} = \mathbf{f}_{0i} + \mathbf{f}_{\Delta i}$, the goal is to find the tendency of change in controls, $\Delta\eta_{i,x}$, $\Delta\eta_{i,y}$, and $\Delta{T_f}_{i}$.
% This problem is solved by linearizing the nonlinear effector model, $\mathbf{f}(\eta_x, \eta_y, T_f)$, w.r.t. the control inputs,
% \begin{align}
%     \mathbf{f}_{i\kappa}
%      & = \mathbf{f}_{i0} + \left.\mathbf{J}_f\right|_{\mathbf{f}_{0i}=\mathbf{f}(\eta_{i,x0}, \eta_{i,y0}, {T_f}_{i0})} \begin{bmatrix}
%                     \Delta \eta_{i,x} \\
%                     \Delta \eta_{i,y} \\
%                     \Delta {T_f}_{i}
%                 \end{bmatrix} \nonumber \\
%      & = \mathbf{f}_{i0} + \kappa  \frac{\mathbf{f}_{\Delta i}}{\|\mathbf{f}_{\Delta i}\|}
%     \label{eq:control:team:CA:tendency_change}
% \end{align}
% where $\kappa$ is a constant, the inverse mapping of $\mathbf{f}(\cdot)$ can be solved using \eqref{eq:control:team:CA:inverse_transform}, and $\mathbf{J}_f$ is the jacobian of $\mathbf{f}(\cdot)$, which is given by
% \begin{align}
%     \mathbf{J}_f & = \left.\begin{bmatrix}
%                                \frac{\partial \mathbf{f}}{\partial \eta_{i,x}} &
%                                \frac{\partial \mathbf{f}}{\partial \eta_{i,y}} &
%                                \frac{\partial \mathbf{f}}{\partial {T_f}_{i}}
%                            \end{bmatrix} \right|_{\mathbf{f}_{0i}=\mathbf{f}(\eta_{i,x0}, \eta_{i,y0}, {T_f}_{i0})} \nonumber       
%                  % & = \begin{bmatrix}
%                  %         - {T_f}_{i0} \sin\eta_{i,x0} \sin\eta_{i,y0} & {T_f}_{i} \cos\eta_{i,x0} \cos\eta_{i,y0}  & \cos\eta_{i,x0} \sin\eta_{i,y0} \\
%                  %         {T_f}_{i} \cos\eta_{i,x0}                    & 0                                          & -\sin\eta_{i,x0}                \\
%                  %         - {T_f}_{i0} \sin\eta_{i,x0} \cos\eta_{i,y0} & -{T_f}_{i} \cos\eta_{i,x0} \sin\eta_{i,y0} & \cos\eta_{i,x0} \cos\eta_{i,y0}
%                  %     \end{bmatrix},
% \end{align}
% where $\mathbf{J}_f$ is non-singular if ${T_f}_i \neq 0$ and $\eta_{i,x0} \neq \pi/2$.
% With the assumption that the initial state is feasible, $\mathbf{f}_{0i} \in \mathcal{D}_i^\star$, the situation of singularity is avoided, and the tendency of changes can be solved by directly inverting \eqref{eq:control:team:CA:tendency_change},
% \begin{equation}
%     \begin{bmatrix}
%         \Delta \eta_{i,x} \\
%         \Delta \eta_{i,y} \\
%         \Delta {T_f}_{i}
%     \end{bmatrix}
%     = \frac{\kappa}{\|\mathbf{f}_{\Delta i}\|}\mathbf{J}_f^{-1} \mathbf{f}_{\Delta i}.
%     \label{eq:control:team:CA:allocation_direction}
% \end{equation}

% =============================================================
\subsection{Intersections on Agent's AFS Boundaries}
Let $\mathcal{D}_i$ be the AFS of agent $i$, given the initial force $\mathbf{f}_{i0}\in \mathcal{D}_i$ and a desired modification $\mathbf{f}_{i\Delta} \in \mathbb{R}^3$. 
The goal is to find a maximum increment $c$ such that $\mathbf{f}_{i0} + c \mathbf{f}_{i\Delta} \in \mathcal{D}_i$, which is illustrated in \figref{fig:control:CA:sol2}.
\begin{figure}[btp] 
    \centering
    \subfloat[\label{fig:control:CA:sol2_sigma_x}]{%
    \includegraphics[width=0.33\linewidth, trim={{1cm} {0.4cm} {1cm} 0}, clip]{imgs/control/team/CA/sol2Fsigma_x.pdf}}
\hfill
    \subfloat[\label{fig:control:CA:sol2_sigma_x}]{%
    \includegraphics[width=0.33\linewidth, trim={{1cm} {0cm} {1.5cm} 0}, clip]{imgs/control/team/CA/sol2Fsigma_y.pdf}}
\hfill
    \subfloat[\label{fig:control:CA:sol2_tf}]{%
    \includegraphics[width=0.33\linewidth, trim={{1cm} {0.5cm} {1cm} 0}, clip]{imgs/control/team/CA/sol2Ftf.pdf}}
\caption{Finding the maximum increment on the AFS boundary. }
\label{fig:control:CA:sol2}
\end{figure}
% the optimization problem is formulated by
% \begin{equation}
%     c_{i\star} = \underset{\mathbf{f}_{i\star}(c) \in \mathcal{D}_i, c>0}{\arg\max}\, \mathbf{f}_{i\star}, \quad \mathbf{f}_{i\star} = \mathbf{f}_{i0}+ c \mathbf{f}_{i\Delta},
%     \label{eq:control:team:CA:maximum_scaling_incre}
% \end{equation}
The problem is solved geometrically by finding the nearest intersection on the three boundaries of $\mathcal{D}_i$.
\begin{equation}
    c_{i\star} = \min\left\{ c_w \middle| c_w > 0, c_w \in \{c_{i,x}, c_{i,y}, c_{i,T_f}, \inf\} \right\}
    \label{eq:ctrl:team:CA:sol2increment_on_boundary},
\end{equation}
where $c_{i,x}$, $c_{i,y}$, and $c_{i,T_f}$ can be solved by establishing
\begin{align*}
    \mathbf{f}_{i0} + c_{i,x} \mathbf{f}_{i\Delta}   & = \mathbf{f}_i(\eta_{i,x}, {\sigma_{y}}, {T_f}_i) \\
    % \label{eq:control:team:sol_to_admis:def_1}        \\
    \mathbf{f}_{i0} + c_{i,y} \mathbf{f}_{i\Delta}   & = \mathbf{f}_i({\sigma_{x}}, \eta_{i,y}, {T_f}_i) \\
    % \label{eq:control:team:sol_to_admis:def_2}        \\
    \mathbf{f}_{i0} + c_{i,T_f} \mathbf{f}_{i\Delta} & = \mathbf{f}_i(\eta_{i,x}, \eta_{i,y}, \sigma_{{T_f}}),
    % \label{eq:control:team:sol_to_admis:def_3}.
\end{align*}
where $\mathbf{f}_i(\cdot)$ is defined by \eqref{eq:model:thrust_force}.
If multiple solutions exist, the smallest one is picked, and thus, $c_{i\star}$ holds a local convexification, i.e., $\mathbf{f}_{i0} + c \mathbf{f}_{i\Delta} \in \mathcal{D}_i, \forall c \in [0, c_{i\star}]$.

% =============================================================
\subsection{Truncated Wrench Allocation (TWA)}\label{sec:CA:EBRWA}
% region [introduction]
% Active agents
Define the sequence of unsaturated agents as 
$% \begin{equation}
    N_\epsilon=\langle N_{\epsilon,i} \in \{0, 1\} | i=1 .. n \rangle \in \mathbb{R}^n,
    \label{eq:model:set_def:active_agents}
$ % \end{equation}
where $N_{\epsilon,i}=1$ indicates an unsaturated agent.
The truncated wrench allocation tries to explore $\mathbf{f}_i$ in  $\mathcal{D}_i$ in all unsaturated agents, i.e., $N_{\epsilon i} \neq 0$.
% endregion [introduction]
% region [truncated effectiveness matrtix]
The truncated effectiveness matrix is formulated by
\begin{equation}
    \mathbf{M}_{\epsilon}(N_\epsilon) := \mathbf{M}(\Xi) (\mathbf{I}_6 \otimes \text{diag}(N_\epsilon)),
    \label{eq:allocation:sat_effectiveness_matrix}
\end{equation}
where $\otimes$ is the Kronecker product. 
% \begin{proposition}
Given $N_\epsilon$ and the desired wrench $\mathbf{u}_\Delta = \mathbf{u}_d - \mathbf{M}\mathbf{f}_0$, the allocation
\begin{equation}
    \mathbf{f}_\Delta = (\mathbf{M}_\epsilon(N_\epsilon))^\dagger  \mathbf{u}_\Delta \in \mathbb{R}^{3n},
    \label{eq:ctrl:team:CA:truncated_allocation}
\end{equation}
satisfies $\mathbf{f}_{i\Delta}=\mathbf{0}, \forall N_{\epsilon, i} = 0$ and $\mathbf{u}_\Delta=\mathbf{M}\mathbf{f}_\Delta$, provided $\text{rank}(\mathbf{M}_\epsilon(N_\epsilon)) \geq 6$ and the weight matrix $\mathbf{W}$ is diagonal and positive-definite, where $(\cdot)^\dagger$ denotes Moore-Penrose pseudoinverse. 
    % \label{prop:control:team:CA:truncated_effectiveness_matrix}
% \end{proposition}
% Proof of \coloredref{Proposition }{prop:control:team:CA:truncated_effectiveness_matrix}:
% With the fact that $\text{rank}(\mathbf{M}^\top \mathbf{M})=\text{rank}(\mathbf{M})=\text{rank}(\mathbf{M}^\top)$, and the condition that $\mathbf{M}_\epsilon$ is full rank, it is clear that $(\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top) \in \mathbb{R}^{6\times 6}$ is invertible.
% By expanding \eqref{eq:allocation:sat_effectiveness_matrix},
% \begin{align*}
%     \mathbf{M}_{\epsilon}(N_\epsilon)
%      & = \begin{bmatrix}
%              \mathbf{M}_1 & \mathbf{M}_2 & \dots & \mathbf{M}_n
%          \end{bmatrix}
%     \text{diag}(N_{\epsilon1}\mathbf{I}_6, N_{\epsilon2}\mathbf{I}_6, \cdots, N_{\epsilon n}\mathbf{I}_6) \\
%      & = \begin{bmatrix}
%              N_{\epsilon1}\mathbf{M}_1 & N_{\epsilon2}\mathbf{M}_2 & \dots & N_{\epsilon n}\mathbf{M}_n
%          \end{bmatrix}.
% \end{align*}
% With $\mathbf{W}=\text{diag}(w_1, w_2, \dots, w_n)$, the weighted pseudo-inverse is
% \begin{align*}
%     \mathbf{M}_\epsilon^\dagger(N_\epsilon)
%      & = \mathbf{W}^{-1}\mathbf{M}^\top (\mathbf{M} \mathbf{W}^{-1} \mathbf{M}^\top)^{-1}
%     = \begin{bmatrix}
%           N_{\epsilon1}/w_1\mathbf{M}_1^\top (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1} \\
%           N_{\epsilon2}/w_2\mathbf{M}_2^\top (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1} \\
%           \vdots                                                                                                 \\
%           N_{\epsilon n}/w_n\mathbf{M}_n^\top (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1}
%       \end{bmatrix}.
% \end{align*}
% It is obvious that if $N_{\epsilon i}=0$, the elements in $i$'th row of $\mathbf{M}_\epsilon^\top(N_\epsilon)$ are all zeros, and therefore, $\mathbf{f}_{\Delta i} = (N_{\epsilon i}/w_i) \mathbf{M}_i^\top (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1} \mathbf{u}_\Delta = \mathbf{0}_3$.
% The effectiveness of the allocation can also be checked by evaluating $\mathbf{u}' = \mathbf{M} \mathbf{M}_\epsilon^\dagger \mathbf{u}_d$.
% With the fact that $\mathbf{W}^{-1}\mathbf{D}^\top = \mathbf{D} \mathbf{W}^{-1} \mathbf{D}^\top$, where $\mathbf{D} = \text{diag}(N_{\epsilon1}\mathbf{I}_6, N_{\epsilon2}\mathbf{I}_6, \cdots, N_{\epsilon n}\mathbf{I}_6)$,
% \begin{align*}
%     \mathbf{u}'
%      & = \mathbf{M} \mathbf{M}_\epsilon^\dagger \mathbf{u}_d                                                                                            \\
%      & = \mathbf{M} \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top  (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1} \mathbf{u}_d          \\
%      & = \mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top  (\mathbf{M}_\epsilon \mathbf{W}^{-1} \mathbf{M}_\epsilon^\top)^{-1} \mathbf{u}_d \\
%      & = \mathbf{u}_d,
% \end{align*}
% which indicates that the truncated allocation generates the desired wrench.

% Considering a 4 agents system as an example, assuming agent 1 and agent 3 are saturated, or $N_\epsilon = \langle 0, 1, 0, 1\rangle$. From \eqref{eq:allocation:sat_effectiveness_matrix}, the truncated effectiveness matrix is
% \begin{equation*}
%     \mathbf{M}_\epsilon(N_\epsilon) = \mathbf{M}(\Xi)
%     \begin{bmatrix}
%         \mathbf{0} & \mathbf{0}   & \mathbf{0} & \mathbf{0}   \\
%         \mathbf{0} & \mathbf{I}_6 & \mathbf{0} & \mathbf{0}   \\
%         \mathbf{0} & \mathbf{0}   & \mathbf{0} & \mathbf{0}   \\
%         \mathbf{0} & \mathbf{0}   & \mathbf{0} & \mathbf{I}_6
%     \end{bmatrix}.
% \end{equation*}
% \todomark{completing the example}
% % endregion [truncated effectiveness matrtix]

% From \coloredref{Remark}{remark:attainable_magnitude_convex}, there must exist a $c_\star$ such that $\mathbf{f}_{o} + c \mathbf{f}_\Delta \in \mathcal{D}^\star, \forall c \in [0, c_\star]$, where $\mathcal{D}^\star = \bigcup_{i=1}^n \mathcal{D}_i^\star$.
Since $\mathbf{f}_0 + \mathbf{f}_\Delta$ may be infeasible, the maximum increment $c_\star$ is chosen to be the smallest $c_{i\star}$ such that at least one agent hits the boundary of its AFS, $\mathcal{D}_i$, or
\begin{equation}
    (c_\star, i_\star) = \arg\min\{c_{i\star} | N_{\epsilon i} = 1, i \in 1..n\},
    % ,\quad i_\star = \underset{i}{\arg\min} c_{i\star}
    \label{eq:allocation:maximum_increment}
\end{equation}
and $i_\star$ is the corresponding saturated agent. 
With the selection of $c_{i\star}$ in \eqref{eq:ctrl:team:CA:sol2increment_on_boundary}, $c_\star$ satisfies $\mathbf{f}_{0} + c \mathbf{f}_\Delta \in \mathcal{D}, \forall c \in [0, c_\star]$, where $\mathcal{D} = \bigcup_{i=1}^n \mathcal{D}_i$.
If $c_\star \geq 1$, the allocation can be completed without saturating any agent.

%% Remark
% Due to the definition of $c_{i\star}$, the solution to $c_{i\star}$ forms a local convex set $\mathcal{D}_{iS}^\star$ on the segment between $\mathbf{f}_{i0}$ and $c_{i\star}\mathbf{f}_{\Delta i}$, i.e., $\mathcal{D}_{iS}^\star = \left\{\lambda_i \mathbf{f}_{i0} + (1-\lambda_i)c_{i\star}\mathbf{f}_{i\Delta} \in \mathcal{D}_i^\star \middle| \forall \lambda_i\in[0,1]\right\} \subset \mathcal{D}_i^\star$.
% The intersection of $\mathcal{D}_{iS}$ for all agent $i$ w.r.t. $c$ is $\mathcal{D}_S^\star = \bigcap_{i=1}^n \mathcal{D}_{iS}^\star = \left\{\lambda\mathbf{f}_0 + (1-\lambda)c_\star \mathbf{f}_\Delta \middle| \forall \lambda\in[0,1]\right\} \subset \mathcal{D}$, which is convex, and thus, any solution in $\mathbf{f}_0+c\mathbf{f}_\Delta, c\in[0, c_\star]$ is feasible.
% Due to the convexity of $\mathcal{D}_i$ in ${T_f}_i$ direction, 

A recursive method to allocate the desired control $\mathbf{u}_d$ by repeatedly finding the increment $c_\star$ proposed in \cite{stephanFastExactRedistributed2019} is adopted but with the allocation function in \eqref{eq:ctrl:team:CA:truncated_allocation} and the maximum increment solved by \eqref{eq:allocation:maximum_increment} and \eqref{eq:ctrl:team:CA:sol2increment_on_boundary} under AFS constraints ${\mathcal{D}}$, provided that initial step $\mathbf{f}_0$ is feasible.
%
In conclusion, one obtains 
\begin{equation*}
    (\mathbf{f}_\text{EBRCA}, c_u) = \text{EBRCA}(\mathbf{u}_d, \mathbf{M}, \mathbf{f}_0, N_\epsilon).
\end{equation*}
The wrench increment $c_u$ satisfies $\mathbf{u}_\text{EBRCA} = c_u (\mathbf{u}_d - \mathbf{u}_0) = \mathbf{M}(\mathbf{f}_\text{EBRCA} - \mathbf{f}_0)$, i.e., finding new allocations in a maximum agility manner \cite{stephanFastExactRedistributed2019}.
% The initial step $\mathbf{f}_0$ is required to be feasible, and $N_{\epsilon0}=\{1, \dots, 1\}$ if no agent disabled.
% Due to the selection of local admissible force space, the initial step $\mathbf{f}_0$ must be feasible 
% The initial step $\mathbf{f}_0$ is required to be feasible, which can be determined by the control at the equilibrium point.  %% TODO: The advantage of choosing the equilibrium point as the initial step
% \begin{algorithm}
%     \caption{Truncated Redistributed Wrench Allocation (TRWA)}\label{alg:truncated_redistributed_alg}
%     \begin{algorithmic}
%         \Require $\mathbf{u}_d \in \mathbb{R}^6$, $\mathbf{M}\in \mathbb{R}^{6\times 3n}$, $\mathbf{f}_0 \in \mathcal{D} \subset \mathbb{R}^{3n \times 1}, N_{\epsilon0} \in \{0, 1\}^n, \mathbf{z}_o \in \mathbb{R}^{4n}$, $c_0 \in [0, 1]$
%         \Ensure $\mathbf{f} \in \mathcal{D}$
%         % \State $\mathbf{f}_0 \gets \mathbf{f}(\mathbf{0}, \mathbf{0}, 1)$
%         % \State $(\eta_{i,x}, \eta_{i,y}, {T_f}_i) = \text{PBP}(\mathbf{z}_o, N_{\epsilon0})$
%         % Solve the local admissible 
%         % \State $(\sigma_{i,x}^\star, \sigma_{i,y}^\star, \sigma_{i,T_f}^\star) \gets \mathcal{D}_i^\star$  \Comment{Refer to \eqref{eq:control:team:CA:interested_boundary}}
%         % \State $\mathbf{u}_0 \gets $ 
%         \State $\mathbf{M}_\epsilon \gets \mathbf{M}(\Xi) (\mathbf{I}_6 \otimes \text{diag}(N_{\epsilon 0}))$
%         \State $k \gets 0$, $c(0) \gets c_0$, $N_\epsilon(0) \gets N_{\epsilon0}$, $\mathbf{u}_\Delta \gets \mathbf{u}_d - \mathbf{M}_\epsilon \mathbf{f}_0$
%         %
%         \While{$c(k) < 1 \cap \text{rank}(\mathbf{M}_\epsilon) \geq 6$}
%         % calculate the truncated effective matrix 
%         \State $\mathbf{M}_\epsilon \gets \mathbf{M}(\Xi) (\mathbf{I}_6 \otimes \text{diag}(N_\epsilon(k)))$
%         \Comment{Refer to \eqref{eq:allocation:sat_effectiveness_matrix}}
%         % calculate new allocations 
%         \State $\mathbf{f}_\Delta \gets \mathbf{M}^\dagger_\epsilon  \mathbf{u}_\Delta$
%         \Comment{Using \coloredref{Proposition}{prop:control:team:CA:truncated_effectiveness_matrix}}
%         %
%         \State Solve $c_{i\star}$
%         \Comment{Using \eqref{eq:ctrl:team:CA:sol2increment_on_boundary}, (\ref{eq:ctrl:team:CA:sol2increment:t_ix}), (\ref{eq:ctrl:team:CA:sol2increment:t_iy}), (\ref{eq:ctrl:team:CA:sol2increment:t_itf})}
%         % solve the maximum increment
%         \State $(c_\star, i_\star) = \arg\min\{c_{i\star} | \forall i \in 1..n, N_{\epsilon i} = 1\}$  \Comment{Refer to \eqref{eq:allocation:maximum_increment}}
%         %
%         \State $N_\epsilon(k+1) \gets N_\epsilon(k) \backslash i_\star$
%         \Comment{Update the saturated agent set. }
%         % determine the maximum increment 
%         \State $d \gets \min(\max(0, c_\star), 1-c(k))$
%         \Comment{To avoid causing $c(k)>1$.}
%         \State $\mathbf{f}(k+1) \gets \mathbf{f}(k) + d \mathbf{f}_\Delta$
%         \State $c(k+1) \gets c(k) + d$
%         \State $k \gets k+1$
%         \EndWhile
%         \State\Return $\mathbf{f}(k), c(k)$
%     \end{algorithmic}
% \end{algorithm}

% =============================================================
% =============================================================
% \subsection{Post-Torque Enhancement}

% % region [why post torque allocation]
% % The nominal force $\tilde{\mathbf{u}}_{fr}$ is typically non-zero due to the gravity.
% % On the contrary, the desired torque control converges to zero if $\mathbf{R}_r$ is stationary.
% %% This requires the condition that the origin of {B} is chosen at CoG of the team
% Large torque allocation errors may appear while encountering high force demands even though the required torque is small.
% Moreover, the desired force realization highly depends on the convergence of a feasible target attitude due to the nature of a \textit{laterally bounded force} system, which also corresponds to the force projection \eqref{eq:fullpose:dir_sat} and the control law \eqref{eq:ctrl:team:lay:control_law}.
% The above-mentioned factors suggest a post-modification to enhance allocation in torque control.
% If $\text{rank}(\mathbf{M}_{\epsilon\tau}(\Xi)) \geq 3$, it suggests that further allocation on torques is possible.
% % \todomark{gives evidence in simulations}
% % endregion [why post torque allocation]

% % region [allocation in null space]
% The idea is to adjust $\mathbf{f}_\text{EBRWA}$ without affecting the force allocation and obey the constraints of LAFS simultaneously.
% By defining the residual torque $\mathbf{u}_{\tau \Delta} = \mathbf{u}_{\tau d} - \mathbf{M}_{\tau} \mathbf{u}_{\tau 0}$, the problem is formulated as
% \begin{align}
%     \mathbf{f}_\Delta = \underset{\mathbf{f}_\Delta \in \mathbb{R}^{3n}}{\arg\max} \left\{
%     c_\tau \in \mathbb{R} \middle|
%     \begin{array}{ll}
%         \mathbf{M}_f \mathbf{f}_\Delta = 0                                                     \\
%         c_\tau \mathbf{u}_{\tau \Delta} = \mathbf{M}_\tau \mathbf{f}_\Delta \\
%         \mathbf{f}_\text{TRWA} + \mathbf{f}_\Delta \in \mathcal{D}^\star \\
%     c_\tau + c_u \leq 1
%     \end{array}
%     \right\},
%     \label{eq:ctrl:team:CA:TPE:prob_formulation}
% \end{align}
% where the solution satisfies 
% \begin{align*}
%     \begin{bmatrix}
%         (c_u + c_\tau)\mathbf{I}_3 & \mathbf{0}_3 \\
%         \mathbf{0}_3 & c_u \mathbf{I}_3
%     \end{bmatrix}
%     (\mathbf{u}_{d} - \mathbf{u}_{0})
%     = \mathbf{M} (\mathbf{f}_\text{EBRWA} + \mathbf{f}_\Delta - \mathbf{f}_0). 
% \end{align*}

% The strategy is to find controls such that $\mathbf{f}_\Delta           = \mathbf{N}_{\mathbf{M}_f} \mathbf{r}$, where $\mathbf{N}_{\mathbf{M}_f} \in \mathbb{R}^{3n \times (3n-3)}$ is the null-space of $\mathbf{M}_f$, and $\mathbf{r} \in \mathbb{R}^{3n-3}$ is an arbitrary vector.
% From the second constraint in \eqref{eq:ctrl:team:CA:TPE:prob_formulation}, one has $c_\tau \mathbf{u}_{\tau \Delta} = \mathbf{M}_\tau \mathbf{N}_{\mathbf{M}_f} \mathbf{r}$, which can be solved by using the Moore-Penrose inverse, or $\mathbf{r} = c_\tau (\mathbf{M}_\tau \mathbf{N}_{\mathbf{M}_f})^\dagger \mathbf{u}_{\tau \Delta}$, and, in consequence, the solution to $\mathbf{f}_\Delta$ is 
% $
% \mathbf{f}_\Delta = \mathbf{N}_{\mathbf{M}_f} (\mathbf{M}_\tau \mathbf{N}_{\mathbf{M}_f})^\dagger \mathbf{u}_{\tau \Delta}.   
% $
% % endregion [allocation in null space]
% % region [Redistributed Iteration]
% Using the same techniques in \secref{sec:CA:EBRWA}, and replacing \eqref{eq:allocation:sat_effectiveness_matrix} and \eqref{eq:ctrl:team:CA:truncated_allocation} with
% \begin{align}
%     \mathbf{M}_{\tau\epsilon}(N_{\tau\epsilon}) & = \mathbf{M}_\tau (\mathbf{I}_3 \otimes \text{diag}(N_{\tau\epsilon})) \mathbf{N}_{\mathbf{M}_f} , \\
%     \mathbf{f}_\Delta                           & = c_\tau \mathbf{N}_{\mathbf{M}_f} \mathbf{M}_{\tau\epsilon}^\dagger(N_{\tau\epsilon}) \mathbf{u}_{\tau \Delta},
%     \label{eq:ctrl:team:CA:PTE:new_allocation}
% \end{align}
% $\mathbf{f}_\Delta$ can be explored in $\mathcal{D}^\star$ in a redistributed manner.
% However, since the direction of allocation, $\mathbf{f}_\Delta$, is not the same as the wrench allocation, the saturated agent set needs to be re-determined.
% Finally, the controls are given by $\mathbf{f}_d = \mathbf{f}_\text{EBRWA} + \mathbf{f}_\text{PTE} + \mathbf{f}_0$.
% % The algorithm for post-torque enhancement is summarized in \coloredref{Algorithm}{alg:PTE_redistributed_alg}.
% % \begin{algorithm}
% %     \caption{Post-Torque Enhancement (PTE)}\label{alg:PTE_redistributed_alg}
% %     \begin{algorithmic}
% %         \Require $\mathbf{u}_{\tau d} \in \mathbb{R}^3$, $\mathbf{M}\in \mathbb{R}^{6\times 3n}$, $\mathbf{f}_0 \in \mathcal{D} \subset \mathbb{R}^{3n \times 1}, N_{\epsilon0} \in \{0, 1\}^n, \mathbf{z}_o \in \mathbb{R}^{4n}$, $c_0 \in [0, 1]$
% %         \Ensure $\mathbf{f} \in \mathcal{D}$
% %         %
% %         \State $\mathbf{M}_{\tau\epsilon} \gets \mathbf{M}_\tau(\Xi) (\mathbf{I}_3 \otimes \text{diag}(N_{\epsilon 0}))$
% %         \State $k \gets 0$, $c(0) \gets c_0$, $N_\epsilon(0) \gets N_{\epsilon0}$, $\mathbf{u}_{\tau\Delta} \gets \mathbf{u}_{\tau d} - \mathbf{M}_{\tau\epsilon} \mathbf{f}_0$
% %         \State $\mathbf{N}_{\mathbf{M}_f} \gets \mathcal{N}(\mathbf{M}_f)$
% %         %
% %         \While{$c(k) < 1 \cap \text{rank}(\mathbf{M}_{\tau\epsilon}) \geq 3$}
% %         % calculate the truncated effective matrix 
% %         \State $\mathbf{M}_{\tau\epsilon} \gets \mathbf{M}_\tau (\mathbf{I}_3 \otimes \text{diag}(N_{\tau\epsilon}(k))) \mathbf{N}_{\mathbf{M}_f}$
% %         % calculate new allocations 
% %         \State $\mathbf{f}_\Delta \gets \mathbf{N}_{\mathbf{M}_f} \mathbf{M}_{\tau\epsilon}^\dagger \mathbf{u}_{\tau \Delta}$
% %         \Comment{Refer to \eqref{eq:ctrl:team:CA:PTE:new_allocation}}
% %         %
% %         \State Solve $c_{i\star}$
% %         \Comment{Using \eqref{eq:ctrl:team:CA:sol2increment_on_boundary}, (\ref{eq:ctrl:team:CA:sol2increment:t_ix}), (\ref{eq:ctrl:team:CA:sol2increment:t_iy}), (\ref{eq:ctrl:team:CA:sol2increment:t_itf})}
% %         % solve the maximum increment
% %         \State $(c_\star, i_\star) = \arg\min\{c_{i\star} | \forall i \in 1..n, N_{\epsilon i} = 1\}$  \Comment{Refer to \eqref{eq:allocation:maximum_increment}}
% %         %
% %         \State $N_\epsilon(k+1) \gets N_\epsilon(k) \backslash i_\star$
% %         \Comment{Update the saturated agent set. }
% %         % determine the maximum increment 
% %         \State $d \gets \min(\max(0, c_\star), 1-c(k))$
% %         \Comment{To avoid causing $c(k)>1$.}
% %         \State $\mathbf{f}(k+1) \gets \mathbf{f}(k) + d \mathbf{f}_\Delta$
% %         \State $c(k+1) \gets c(k) + d$
% %         \State $k \gets k+1$
% %         \EndWhile
% %         \State\Return $\mathbf{f}(k), c(k)$
% %     \end{algorithmic}
% % \end{algorithm}
% % endregion [Redistributed Iteration]



% \subsection{Inverse Mapping\label{sec:contro:team:CA:inverse_mapping}}
Finally, recalling the definition of $\mathbf{f}_i$ in \eqref{eq:model:team:effectiveness_model}, the inverse mapping of $\mathbf{f}_{id}$ is
\begin{align}
    \begin{cases}
        {T_f}_{id}  = \|\mathbf{f}_{id}\|_2,          \\
        \eta_{i,xd} = \arcsin\left(
        \frac{-\mathbf{f}_{id,y}}{{T_f}_{id}}\right), \\
        \eta_{i,yd} = \arctan2\left(
        \frac{\mathbf{f}_{id,x}}{\text{sgn}(\cos\eta_{i,xd})},
        \frac{\mathbf{f}_{id,z}}{\text{sgn}(\cos\eta_{i,xd})}\right).
    \end{cases}
\end{align}
% To eliminate the actuator baud-rate attenuation \cite{oppenheimerMethodsCompensatingControl2004} induced by CA, a feedforward compensator is used
% \begin{equation}
%     \mathbf{z}_{id} = \begin{bmatrix}
%         k_{zx} \mathbf{I}_2 & 
%         k_{zv} \mathbf{I}_2 & 
%         \mathbf{0}_2
%     \end{bmatrix} \mathbf{z}_i + 
%     k_{zff} \begin{bmatrix}
%         \eta_{i,xd} \\ \eta_{i,yd}
%     \end{bmatrix},
% \end{equation}
% which completes the control allocation.
% The overall algorithm of the proposed exact bundled redistributed control allocation is summarized in \coloredref{Algorithm}{alg:redistributed_alg}.
% \begin{algorithm}
%     \caption{Exact Bundled Redistributed Allocation (EBRA)}\label{alg:redistributed_alg}
%     \begin{algorithmic}
%         \Require $\mathbf{u}_d \in \mathbb{R}^6$, $\mathbf{M}\in \mathbb{R}^{6\times 3n}$, $\mathbf{f}_0 \in \mathcal{D} \subset \mathbb{R}^{3n \times 1}, N_{\epsilon0} \in \{0, 1\}^n, \mathbf{z}_o \in \mathbb{R}^{4n}$
%         \Ensure $\mathbf{f} \in \mathcal{D}$
%         % PBP
%         \State $\mathcal{D}_i' = \text{PBP}(\mathbf{f}_0, \mathbf{z}_o, N_{\epsilon0})$
%         \Comment{Refer to \eqref{eq:control:team:CA:pseudo_boundary_space}}
%         \State $\mathbf{f}_0 = {\text{clip}}_{\mathcal{D}_i'}(\mathbf{f}_0)$
%         % local admissible 
%         % \State $(\sigma_{i,x}^\star, \sigma_{i,y}^\star, \sigma_{i,T_f}^\star) \gets \mathcal{D}_i^\star$  \Comment{Refer to \eqref{eq:control:team:CA:interested_boundary}}
%         % intersection
%         \State $\mathcal{D}_i^\star \gets \text{LocalAdmissibleForceSpace}(\mathbf{f}_0, \mathbf{f}_\Delta, \kappa)$
%         \Comment{Refer to \eqref{eq:control:team:CA:local_admissible_force_set}}
%         % wrench allocation
%         \State $(\mathbf{f}_\text{TRWA}, c_u) \gets \text{TRWA}(\mathbf{u}_d, \mathbf{M}, \mathbf{f}_0, N_{\epsilon 0}, \mathbf{z}_o, 0)$

%         \State $(\mathbf{f}_\text{EBRA}, c_\tau) \gets \text{PTE}(\mathbf{u}_d, \mathbf{M}, \mathbf{f}_0, N_{\epsilon 0}, \mathbf{z}_o, c_u)$

%         \State $(\eta_{id,x}, \eta_{id,y}, {T_f}_{id}) \gets \mathbf{f}^{-1}(\mathbf{f}_{\text{EBRA},i}), \forall i \in 1..n$
%         \Comment{Refer to \eqref{eq:control:team:CA:inverse_transform}}
%         \State\Return $(\eta_{id,x}, \eta_{id,y}, {T_f}_{id})$
%     \end{algorithmic}
% \end{algorithm}

==> front/abstract.tex <==
% !TeX root = ../main.tex

\begin{abstract}

    \begin{tempsection}
        中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要中文摘要
    \end{tempsection}

\end{abstract}

\begin{abstract*}

    \begin{tempsection}
        Abstract
    \end{tempsection}

\end{abstract*}

==> front/acknowledgement.tex <==
% !TeX root = ../main.tex

\begin{acknowledgement}

\begin{tempsection}
常到外國朋友家吃飯。當蠟燭燃起，菜肴布好，客主就位，總是主人家的小男孩或小女孩舉起小手，低頭感謝上天的賜予，並歡迎客人的到來。

我剛到美國時，常鬧得尷尬。因為在國內養成的習慣，還沒有坐好，就開動了。

以後凡到朋友家吃飯時，總是先囑咐自己；今天不要忘了，可別太快開動啊！幾年來，我已變得很習慣了。但我一直認為只是一種不同的風俗儀式，在我這方面看來，忘或不忘，也沒有太大的關係。

前年有一次，我又是到一家去吃飯。而這次卻是由主人家的祖母謝飯。她雪白的頭髮，顫抖的聲音，在搖曳的燭光下，使我想起兒時的祖母。那天晚上，我忽然覺得我平靜如水的情感翻起滔天巨浪來。

在小時候，每當冬夜，我們一大家人圍著個大圓桌吃飯。我總是坐在祖母身旁。祖母總是摸著我的頭說：「老天爺賞我們家飽飯吃，記住，飯碗裡一粒米都不許剩，要是蹧蹋糧食，老天爺就不給咱們飯了。」

剛上小學的我，正在念打倒偶像及破除迷信等為內容的課文，我的學校就是從前的關帝廟，我的書桌就是供桌，我曾給周倉畫上眼鏡，給關平戴上鬍子，祖母的話，老天爺也者，我覺得是既多餘，又落伍的。

不過，我卻很尊敬我的祖父母，因為這飯確實是他們掙的，這家確實是他們立的。我感謝面前的祖父母，不必感謝渺茫的老天爺。

這種想法並未因為年紀長大而有任何改變。多少年，就在這種哲學中過去了。

我在這個外國家庭晚飯後，由於這位外國老太太，我想起我的兒時，由於我的兒時，我想起一串很奇怪的現象。

祖父每年在「風裡雨裡的咬牙」，祖母每年在「茶裡飯裡的自苦」，他們明明知道要滴下眉毛上的汗珠，才能撿起田中的麥穗，而為什麼要謝天？我明明是個小孩子，混吃混玩，而我為什麼卻不感謝老天爺？

這種奇怪的心理狀態，一直是我心中的一個謎。

一直到前年，我在普林斯頓，瀏覽愛因斯坦的我所看見的世界得到了新的領悟。

這是一本非科學性的文集，專載些愛因斯坦在紀念會上啦，在歡迎會上啦，在朋友的喪禮中，他所發表的談話。

我在讀這本書時忽然發現愛因斯坦想盡量給聽眾一個印象：即他的貢獻不是源於甲，就是由於乙，而與愛因斯坦本人不太相干似的。

就連那篇亙古以來嶄新獨創的狹義相對論，並無參考可引，卻在最後天外飛來一筆，「感謝同事朋友貝索的時相討論。」

其他的文章，比如奮鬥苦思了十幾年的廣義相對論，數學部份推給了昔年好友的合作：這種謙抑，這種不居功，科學史中是少見的。

我就想，如此大功而竟不居，為什麼？像愛因斯坦之於相對論，像我祖母之於我家。

幾年來自己的奔波，做了一些研究，寫了幾篇學術文章，真正做了一些小貢獻以後，才有了一種新的覺悟：即是無論什麼事，得之於人者太多，出之於己者太少。因為需要感謝的人太多了，就感謝天罷。無論什麼事，不是需要先人的遺愛與遺產，即是需要眾人的支持與合作，還要等候機會的到來。越是真正做過一點事，越是感覺自己的貢獻之渺小。

於是，創業的人，都會自然而然的想到上天，而敗家的人卻無時不想到自己。

\end{tempsection}

\end{acknowledgement}

==> front/denotation.tex <==
% !TeX root = ../main.tex

\begin{denotation}[3cm]

\item[HPC]{
  高性能計算 (High Performance Computing)
}

\item[cluster]{
  集群
}

\item[Itanium]{
  安騰
}

\item[SMP]{
  對稱多處理
}

\item[API]{
  應用程序編程接口
}

\item[PI]{
  聚酰亞胺
}

\item[MPI]{
  聚酰亞胺模型化合物，N-苯基鄰苯酰亞胺
}

\item[PBI]{
  聚苯並咪唑
}

\item[MPBI]{
  聚苯並咪唑模型化合物，N-苯基苯並咪唑
}

\item[PY]{
  聚吡嚨
}

\item[PMDA-BDA]{
  均苯四酸二酐與聯苯四胺合成的聚吡嚨薄膜
}

\item[$\Delta G$]{
  活化自由能 (Activation Free Energy)
}

\item[$\chi$]{
  傳輸系數 (Transmission Coefficient)
}

\item[$E$]{
  能量
}

\item[$m$]{
  質量
}

\item[$c$]{
  光速
}

\item[$P$]{
  概率
}

\item[$T$]{
  時間
}

\item[$v$]{
  速度
}

\item[勸學]{
  君子曰：學不可以已。青，取之於藍，而青於藍；冰，水為之，而寒於水。木直中繩。輮以為輪，其曲中規。雖有槁暴，不覆挺者，輮使之然也。故木受繩則直，金就礪則利，君子博學而日參省乎己，則知明而行無過矣。吾嘗終日而思矣，不如須臾之所學也；吾嘗跂而望矣，不如登高之博見也。登高而招，臂非加長也，而見者遠；順風而呼，聲非加疾也，而聞者彰。假輿馬者，非利足也，而致千裏；假舟楫者，非能水也，而絕江河，君子生非異也，善假於物也。積土成山，風雨興焉；積水成淵，蛟龍生焉；積善成德，而神明自得，聖心備焉。故不積跬步，無以至千裏；不積小流，無以成江海。騏驥一躍，不能十步；駑馬十駕，功在不舍。鍥而舍之，朽木不折；鍥而不舍，金石可鏤。蚓無爪牙之利，筋骨之強，上食埃土，下飲黃泉，用心一也。蟹六跪而二螯，非蛇鱔之穴無可寄托者，用心躁也。—— 荀況
}

\end{denotation}

